Deep Binarized Photonic Reservoir Computing for Ultrafast Multimedia Signal Processing

We present a deep photonic neural network architecture based on ultrafast binary optical modulation from a digital micro-mirror device (DMD), optical scattering in random medium, high-speed photodetection with a CMOS sensor, and time-multiplexed deep layer structure. Operating at Gigabit-per-second (Gb/s) processing rates, our system based on the reservoir computing (RC) framework achieves state-of-the-art performance across various multimedia tasks, including video, image and speech recognition. We show that the careful optimization of key physical intra- and inter-layer hyper-parameters can significantly enhance the deep photonic RC system ability to extract relevant temporal and spatial features via balancing memory retention and dynamical response of individual layers. This approach paves the way for highly scalable hierarchical photonic reservoir computing systems for high-throughput real-time multimedia signal processing.

==> temp.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{0.9}
\begin{threeparttable}
\caption{Comparison of our binarized deep photonic reservoir computing system with representative state-of-the-art digital and hardware-based approaches on KTH, MNIST, and TI-46 tasks. The selection highlights recent and relevant works for each benchmark.}
\label{table:Performance_compairson_table}
\begin{tabular}{
    >{\centering\arraybackslash}m{0.8cm} % Task column
    >{\centering\arraybackslash}m{3.5cm} % Publication
    >{\centering\arraybackslash}m{5.5cm} % Method + preprocessing
    >{\centering\arraybackslash}m{1.8cm} % Network Size
    >{\centering\arraybackslash}m{1.5cm} % Proc. speed
    >{\centering\arraybackslash}m{1.5cm} % Accuracy
}

\rowcolor{headerblue}
\textbf{Task} & \textbf{Publication} & \textbf{Method + Preprocessing} & \textbf{Network Size} & \textbf{Proc. Speed (f.p.s.)} & \textbf{Accuracy (\%)} \\
\midrule

% KTH block
\multirow{17}{*}{\boxedrotate{2cm}{KTH}} 
& Jaouedi et al. (2020)\cite{jaouedi_new_2020} 
& GRNN with motion tracking, GMM + KF feature extraction, and input frame selection 
& - & - &  \shortstack{FD 96.30 \vspace{0.3em}\\ S1 \makebox[3em]{--}} \\
& \cellcolor{lightblue}Sharif et al. (2017)\cite{sharif_framework_2017} 
& \cellcolor{lightblue}Multi-class SVM with feature extraction (HOG, LBP, texture) and feature selection (Euclidean, min. dist, joint entropy) 
& \cellcolor{lightblue}- & \cellcolor{lightblue}10  & \cellcolor{lightblue}\shortstack{FD 99.30 \vspace{0.3em}\\ S1 \makebox[3em]{--}} \\
& Khan et al. (2021)\cite{khan_resource_2021}
& 26-layer Deep CNN with Poisson distribution and univariate measures (PDaUM) preprocessing 
& \inlineTilde 195 million & - & \shortstack{FD 98.30 \vspace{0.3em}\\ S1 \makebox[3em]{--}} \\
& \cellcolor{lightblue}Shu et al. (2014)\cite{shu_bio-inspired_2014} 
& \cellcolor{lightblue}Bio-inspired SNN with preprocessing 
& \cellcolor{lightblue}24000 & \cellcolor{lightblue}- & \cellcolor{lightblue}\shortstack{FD 92.30 \vspace{0.3em}\\ S1 \makebox[3em]{95.30}} \\
& Picco et al. (2023)\cite{picco_high_2023}
& TDRC with silhouette segmentation, keyframe selection, HOG, PCA preprocessing 
& - & 160  & \shortstack{FD 90.83 \vspace{0.3em}\\ S1 \makebox[3em]{96.67}} \\
& \cellcolor{lightblue}Antonik et al. (2019)\cite{antonik2019human}
& \cellcolor{lightblue}Photonic RC with HOG + PCA preprocessing 
& \cellcolor{lightblue}16384 & \cellcolor{lightblue}2–7  & \cellcolor{lightblue}\shortstack{FD \makebox[2em]{--} \vspace{0.2em}\\ S1 \makebox[2.5em]{91.30}} \\
& \textbf{This work}
& \textbf{Binarized deep photonic RC with HOG + PCA }
& \textbf{10000} & \textbf{\inlineTilde 1000 } & \textbf{\shortstack{FD \makebox[2em]{--} \vspace{0.2em}\\ S1 \makebox[2.5em]{96.67}}} \\

\midrule

% MNIST block
\multirow{10}{*}{\boxedrotate{2cm}{MNIST}} 
& Yepes et al. (2017)\cite{yepes_improving_2017}
& SNN deployed on IBM TrueNorth chip 
& - & - & 98.00 \\
& \cellcolor{lightblue}Wang et al. (2025)\cite{wang_asymmetrical_2025}
& \cellcolor{lightblue}Deep photonic NN with asymmetrical training on PICs; PCA reduces 784 features to 8 
& \cellcolor{lightblue}- & \cellcolor{lightblue}- & \cellcolor{lightblue}95.80 \\
& Du et al. (2017)\cite{du2017reservoir}
& Memristor-based RC hardware 
& 88 memristors & - & 88.10 \\
& \cellcolor{lightblue}Talukder et al. (2025)\cite{talukder_spiking_2025}
& \cellcolor{lightblue}Spiking photonic NN trained on \inlineTilde 6000 images 
& \cellcolor{lightblue}40000 & \cellcolor{lightblue}- & \cellcolor{lightblue}83.50 \\
& Han et al. (2020)\cite{han_hardware_2020} 
& SNN implemented on FPGA 
& 16384 & 161  & 97.06 \\
& \cellcolor{lightblue}\textbf{This work} 
& \cellcolor{lightblue}\textbf{Binarized deep photonic RC with HOG + PCA} 
& \cellcolor{lightblue}\textbf{\inlineTilde 2000} & \cellcolor{lightblue}\textbf{\inlineTilde 1000 } & \cellcolor{lightblue}\textbf{96.36} \\

\midrule

% TI-46 block
\multirow{12}{*}{\boxedrotate{2cm}{TI-46}} 
& Zheng et al. (2021)\cite{zheng_parameters_2021}
& TDRC with nonlinear Duffing oscillator; preprocessing includes Lyon cochleagram 
& 100 & - & 99.80 \\
& \cellcolor{lightblue}Pico et al. (2025)\cite{picco_deep_2025} 
& \cellcolor{lightblue}Deep photonic RC with CMA-ES evolutionary algorithm; Lyon cochleagram preprocessing 
& \cellcolor{lightblue}600 & \cellcolor{lightblue}- & \cellcolor{lightblue}99.40 \\
& Paquot et al. (2012)\cite{paquot2012optoelectronic}
& Optoelectronic RC with Lyon cochleagram preprocessing 
& 200 & - & 99.60 \\
& \cellcolor{lightblue}Wan et al. (2025)\cite{wan_reservoir_2025} 
& \cellcolor{lightblue}TDRC system based on polymer electrolyte-gated MoS$_2$ transistors 
& \cellcolor{lightblue}- & \cellcolor{lightblue}- & \cellcolor{lightblue}95.10 \\
& Zhong et al. (2021)\cite{zhong2021dynamic}
& Dynamic memristor-based RC with Lyon cochleagram preprocessing 
& 400 & - & 99.60 \\
& \cellcolor{lightblue}\textbf{This work} 
& \cellcolor{lightblue}\textbf{Binarized deep photonic RC with Lyon cochleagram preprocessing} 
& \cellcolor{lightblue}\textbf{300} & \cellcolor{lightblue}\textbf{\inlineTilde 1000 } & \cellcolor{lightblue}\textbf{100.00} \\

\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[‡]Network size and processing speed is either not mentioned explicitly or hard to determine. Additionally, accuracy values are reported from the original publications. 
\item[‡]Various abbreviations: FD - Full dataset, S1 - Scenario 1 of KTH dataset, GRNN - Gated Recurrent Neural Network, GMM - Gaussian mixture model, KF - Kalman filter, SVM - Support vector machines, HOG - Histogram of gradients, CNN - Convolutional Neural Network, SNN - Spiking Neural Networks, TDRC - Time delay reservoir computer, PCA - principle component analysis, PICs - photonic integrated circuits, FPGA - Field-Programmable Gate Arrays, CMA-ES - covariance matrix adaption-evolution strategy.
\end{tablenotes}
\end{threeparttable}
\end{table}

% old abstract

We present a deep photonic neural network architecture based on ultrafast binary optical modulation from a digital micro-mirror device (DMD), optical scattering in random medium,  high-speed photodetection with a CMOS sensor, and time-multiplexed deep layer structure. Operating at Gigabit-per-second processing rates, our system based on the reservoir computing (RC) framework achieve state-of-the-art performance across various multimedia tasks, with classification accuracy of $99\%$ for the TI-46 database (speech recognition), $96\%$ for MNIST (image recognition), and $97\%$ for KTH database (human action recognition). We show that optimization of key physical hyper-parameters (\emph{e.g.} leaky rates, neurons per layer...) can enhance our system’s ability to extract relevant temporal and spatial features by balancing memory retention and dynamical response. Binary optical modulation not only enhances computational speed and robustness but also enables efficient optical encoding, reducing power consumption and hardware complexity compared. This approach paves the way for highly scalable hierarchical photonic reservoir computing systems for high-throughput real-time multimedia signal processing.
